Inst3D-LMM: Instance-Aware 3D Scene Understanding with Multi-modal Instruction Tuning

Despite encouraging progress in 3D scene understanding, it remains challenging to develop an effective Large Multi-modal Model (LMM) that is capable of understanding and reasoning in complex 3D environments. Most previous methods typically encode 3D point and 2D image features separately, neglecting interactions between 2D semantics and 3D object properties, as well as the spatial relationships within the 3D environment. This limitation not only hinders comprehensive representations of 3D scene, but also compromises training and inference efficiency. To address these challenges, we propose a unified Instance-aware 3D Large Multi-modal Model (Inst3D-LMM) to deal with multiple 3D scene understanding tasks simultaneously. To obtain the fine-grained instance-level visual tokens, we first introduce a novel Multi-view Cross-Modal Fusion (MCMF) module to inject the multi-view 2D semantics into their corresponding 3D geometric features. For scene-level relation-aware tokens, we further present a 3D Instance Spatial Relation (3D-ISR) module to capture the intricate pairwise spatial relationships among objects. Additionally, we perform end-to-end multi-task instruction tuning simultaneously without the subsequent task-specific fine-tuning. Extensive experiments demonstrate that our approach outperforms the state-of-the-art methods across 3D scene understanding, reasoning and grounding tasks. Source code is available at https://github.com/hanxunyu/Inst3D-LMM

==> sec/1_intro_backup.tex <==
\section{Introduction}
\label{sec:intro}



Building Large Multi-modal Models (LMMs) for 3D scene understanding becomes an emerging research topic with significant potential for advancing robotics~\cite{rana2023sayplan}. For example, the interactive embodied agents~\cite{song2023llm} are expected to interpret 3D layouts and predict object locations based on human instructions.

Traditional 3D scene understanding methods \cite{ma2022sqa3d,wu2023eda} are typically tailored for individual downstream tasks, such as 3D Visual Grounding (3D-VG), 3D Question Answering (3D-QA) and 3D Dense Captioning (3D-DC). 
In contrast, LMMs are able to handle various 3D perception tasks within a single model.
Some methods~\cite{hong20233d,zhu2024empowering} primarily focus on translating 3D points into the space of 2D Vision Language Models (VLMs) and aggregating multi-view features for 3D representations. Alternatively, some approaches~\cite{chen2024ll3da,chen2024grounded} directly encode the features of 3D points and facilitate visual interactions using 3D-text data. 
% They normally utilize unique object identifiers or referent tokens to simplify textual queries and reduce ambiguity in multi-turn conversations. 
% Despite the notable success of existing scene-level LMMs in understanding 3D world with natural language
\textbf{Despite their notable successes, }
% , they behave optimal performance in capturing fine-grained instance-level 3D object features and 
\textbf{existing methods typically require multi-stage alignment or language-scene pre-training, and fail to capture fine-grained instance-level 3D object features, which hampers training efficiency and complicates the development of a versatile model capable of handling multiple tasks.} 
Moreover, two critical challenges for 3D LMMs still remain: 1) \textit{how to effectively integrate 3D object properties, such as geometric and semantics, into LLMs?} and 2) \textit{how to accurately capture the intricate spatial relationships between objects in 3D environments?} These challenges also limit the scope of dialogue content for 3D LMMs and pose obstacles in tackling complex and open-ended tasks in real-world applications.







To address the above issues,  we propose Inst3D-LMM, a unified \textbf{Inst}ance-aware \textbf{3D} \textbf{L}arge \textbf{M}ulti-modal \textbf{M}odel that tackles multiple 3D-language tasks without resorting to task-specific fine-tuning. 
% (VFMs) in conjunction with LLM to  
\textbf{In contrast to previous approaches, Inst3D-LMM fully leverages the powerful 2D Vision Foundation Models (VFMs) and 3D specialist models to }
%the rapid advancement of existing powerful foundation models, such as 2D VFMs and 3D models, has made it possible to efficiently 
\textbf{extract 2D and 3D features at instance-level respectively, which can effectively eliminate confusion arising from vague text descriptions and enhance the identification of objects corresponding to complex descriptions. }
Our approach generates fine-grained instance-level representations that comprehensively encapsulate geometric and semantic properties while capturing intricate pairwise spatial relationships among objects in a 3D scene. By following this instance-aware methodology, our Inst3D-LMM significantly improves the  LLM's ability to accurately comprehend 3D scenes.

Specifically, 
% unlike 3D point clouds data, 2D image data offers rich semantic information that can supplement various attributes of a 3D scene, such as textures, affordances, material properties and situational context. Thus, 
we begin by extracting instance-level 3D features using pre-trained 3D specialist models along with their enriched multi-view 2D semantic features by 2D VFMs, such as SAM~\cite{kirillov2023segment} and CLIP~\cite{radford2021learning}. 
To generate fine-grained instance-level representations integrating both 3D geometric and 2D semantic properties, we introduce a novel Multi-view Cross-Modal Fusion (MCMF) module to effectively infuse enriched multi-view   
%from contextual open-vocabulary 
2D features into the original 3D features with coarse semantic representation. 
A learnable \texttt{[CLS]} token is introduced to aggregate the characteristics of each 2D view and perform this process efficiently.
%to produce fine-grained instance-level representations. 
In order to capture intricate pairwise spatial relationships between objects in a 3D scene, we devise the 3D Instance Spatial Relation (3D-ISR) module that leverages a spatial condition self-attention operation between manifold position embeddings and instance-level visual tokens to produce relation-aware scene-level representations. The resulting instance-level and scene-level representations are subsequently fed into the LLM to enable end-to-end multi-task instruction tuning.

Extensive experiments across various tasks, including 3D-VG, 3D-QA and 3D-DC, demonstrate that our approach outperforms previous state-of-the-art methods with leading 3D scene understanding, grounding and reasoning capabilities. In contrast to most existing methods that focus on close-set scene understanding or require per-task fine-tuning, our Inst3D-LMM operates as a generalist model. We believe this work lays a fundamental step towards unifying diverse 3D vision-language tasks within generative language modeling.


To summarize, our contributions are as follows:
\begin{itemize}
    \item We propose a unified instance-aware LLM-based framework, called Inst3D-LMM for various 3D scene understanding tasks with end-to-end multi-modal instruction tuning. Serving as a generalist model, our approach demonstrates superior performance in 3D scene understanding\&reasoning and spatial localization.
    % Distinguishing itself from other 3D-LLMs, our method 
    % functions as a generalist model, eliminating the necessity for task-specific fine-tuning across various downstream tasks.
    \item We utilize 2D VFMs to extract mutli-view contextual features for each 3D instance and then devise a Multi-view Cross-Modal Fusion (MCMF) module to effectively enhance instance-level feature representations by jointly integrating 3D geometry and 2D semantic priors.
    \item 
    %Based on fused 3D visual tokens output from MCMF, 
    A 3D Instance Spatial Relation (3D-ISR) module is introduced to boost the capability of LMM in understanding the complex spatial details within 3D scenes. 
    %Through the collaboration of MCMF and 3D-ISR, 
    %we effectively inject the instance-level 3D information into LLMs.
\end{itemize}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}
% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/3_methodology_backup.tex <==
\section{Methodology}

% 最好补一下对任务整体的介绍（输入输出）
% \subsection{Overview}
% In our framework, inputs consist of point clouds representing the 3D scene and corresponding RGB-D image frames. 
Our goal is to enable LLM to understand the 3D environment and perform various visual interaction tasks according to human instructions. 
Figure~\ref{pipeline} illustrates the architecture of our framework. For each 3D scene, we employ point clouds and their corresponding RGB-D images as the visual inputs.
In this section, we first introduce how to extract the features at the instance level using pre-trained 3D models~\cite{schult2023mask3d,zhou2023uni3d} and 2D VFMs~\cite{kirillov2023segment,radford2021learning}, respectively. Secondly, we present a novel Multi-view Cross-Modal Fusion (\textbf{MCMF}) module to obtain the fine-grained instance-level tokens, which is specially designed to effectively integrate 3D geometric features with their corresponding multi-view 2D semantic features. Thirdly, we introduce the 3D Instance Spatial Relation (\textbf{3D-ISR}) module to enhance LLM's ability to capture spatial information at the scene level, which generates the relation-aware tokens by calculating the attention scores with respect to the spatial relationships between different 3D instance proposals. 
Under our proposed framework, the MCMF and 3D-ISR modules are jointly optimized so that they can collaboratively benefit each other. 
%in our unified framework. 
Finally, we conduct end-to-end multi-task instruction tuning for different 3D scene understanding tasks simultaneously.

\subsection{Instance-Level Feature Extraction}
\noindent \textbf{3D Feature Extraction.} We first segment the 3D point clouds of each individual instance in a \textit{class-agnostic} manner by leveraging a pre-trained 3D instance segmentation model~\cite{schult2023mask3d}. 
% To break the boundaries of closed-vocabulary semantic predictions, 
We only retain the predicted binary 3D instance masks while ignoring their closed-vocabulary class labels. All instance proposals in one scene are represented by $O^{3D}=\left( O_{1}^{3D}, \ldots, O_{N}^{3D} \right)$, where $O_{i}^{3D}=[coordinate,color]$ consists of the attributes of each instance. We obtain all instance proposals of a scene, and the pre-trained 3D encoder $\mathbf{E_{o}}$~\cite{zhou2023uni3d} is used to extract their instance-level features, \textit{i.e.}, $\mathbf{f_{o}^{3D}} = \mathbf{E_{o}}\left(O^{3D}\right)$.
\\
\noindent \textbf{2D Feature Extraction.} Due to the inherent sparsity of 3D point cloud data, the previous methods have difficulties in generating discriminative features of each object. In this work, we employ powerful 2D VFMs to extract 2D semantic features for each 3D instance. 
As in~\cite{takmaz2023openmask3d,cao2024coda}, we firstly project the point cloud of each instance $O_{i}^{3D}$ onto the image plane and then select the top $K$ views according to the number of visible points. To obtain the accurate 2D masks, we randomly sample $\mathit{k}_{\text{sample}}=5$ points as the input prompts for SAM~\cite{kirillov2023segment} to deal with noisy bounding boxes with outliers. Hereby, we select the high-quality mask with the highest confidence score. To enrich features with contextual information, these masks are employed to generate multi-level ($\mathit{L}$) crops of the selected images that are further fed into the pre-trained CLIP vision encoder ~\cite{radford2021learning} to extract features with language-aligned embedding space. Finally, we aggregate multi-level features of sub-images from the same frame to form the 2D multi-view features $O^{2D}$. 


\begin{figure}[t]
    % \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth]{figures/MCMF-new.pdf}
        \caption{Architecture of the proposed Multi-view Cross-Modal Fusion (MCMF) module.}
        \label{MCMF_module}
        \vspace{-4.8mm}
    % \end{minipage}%
\end{figure}






\subsection{Multi-view Cross-Modal Fusion (MCMF)}
To better fuse 3D geometry priors with 2D multi-view semantic priors, we introduce an effective Multi-view Cross-Modal Fusion (MCMF) module that generates the enriched token representations for each 3D instance before being fed into LLM. The architecture of MCMF is crafted with a coarse-to-fine framework, as shown in Figure~\ref{MCMF_module}.
To map 3D object features $O^{3D}\in \mathbb{R}^{1 \times N \times {D^{3d}}}$ and 2D CLIP features $O^{2D} \in \mathbb{R}^{K \times N \times {D^{2d}}}$ into the embedding space of LLM with the dimensionality of $D$, we utilize a simple two-layer MLP with a LayerNorm and GELU in between, yielding  $O^{3D'}$ and $O^{2D'}$, respectively. $N$ represents the number of instances, and $K$ is the number of images for each object.

Subsequently, we introduce a Cross-Modal Injection Block to transform the enriched semantic priors from 2D multi-view representations into 3D instance features. 
Moreover, we adopt a straightforward self-attention layer to further enhance such 3D instance features. For 2D multi-view features, we append a learnable \texttt{[CLS]} token $t_k$ to the flattened CLIP feature maps in order to adaptively encapsulate the global semantic representation of the $k$-th view. Then, we apply a self-attention layer to multi-view features, enabling semantic gathering to derive $t_{k}^{'}$ for $k$-th view as:
%use the output $t_{k}^{'}$ to represent the global feature of the $k$ view of the instance as:
\begin{equation}
    t_{k}^{'} = \phi(\text{SelfAttn}([t_k, O_{\text{view}\_k}^{2D'}])),
\end{equation}
where $1 \leq k \leq K$, %$t$ is the learnable embedding, 
$O_{\text{view}\_k}^{2D'} \in \mathbb{R}^{ N \times {D}}$. $\phi$ is an indicator function that outputs the updated \texttt{[CLS]} token as the first one from the token list.

\begin{figure}[t]
    % \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=1.0\linewidth]{figures/3D-ISR-new.pdf}
        % \includegraphics[width=\textwidth]{figures/3D-ISR.pdf}
        \caption{Illustration of the 3D Instance Spatial Relation (3D-ISR) module in our framework.}
        \label{3D-ISR}
        \vspace{-4mm}
    % \end{minipage}%
\end{figure}

We obtain the processed 3D token embedding $O^{3D'}\in \mathbb{R}^{1 \times N \times D}$ containing coarse semantics, where each instance in $O^{3D'}$ corresponds to multiple views of the processed 2D CLIP features $O^{2D'}$. It can be represented as follows:
\begin{equation}
   O_i^{2D'} = \left[ t_1', \ldots, t_K' \right], \quad i \in [1, N].
\end{equation}
To infuse the enriched semantic 2D features into 3D geometric feature, we construct the 3D-to-2D-Multi-view pairs, \textit{i.e.} each 3D instance feature in $O^{3D'}\in \mathbb{R}^{1 \times N \times D}$ corresponds to 2D features across $K$ views in $O^{2D'}\in \mathbb{R}^{K \times N \times D}$. In particular, we utilize the preliminary $O^{3D'}$ as queries, while the 2D multi-view visual features $O^{2D'}$ as enriched reference keys and values. 
The injection process is conducted via a cross-attention layer, which encourages  3D instance queries to absorb the fine-grained semantics of keys and values. This results in the enhanced 3D instance features $O^{3D}_{f} \in \mathbb{R}^{1 \times N \times D}$ as below:
\begin{equation}
    O_{f}^{3D} = \text{CrossAttn}(O^{3D'},O^{2D'}).
\end{equation}
%we devise an injection module to enhance and update the original 3D instance representations. 
% that can be regarded as the coarse representations,
% and a self-attention mechanism to get $O^{3D'}$ and $O_{views}^{2D}$ as:\begin{gather}
%     O^{3D'} = \text{SelfAttn}(\text{MLP}(O^{3D})),\\
%     O_{views}^{2D} = \text{MLP}(O^{2D}).
% \end{gather}
Furthermore, we leverage a residual operation by adding the input $O^{3D'}$ to retain the basic characteristics in generating the instance-level 3D visual tokens, $O_{I}^{3D} = O_{f}^{3D} + O^{3D'}$.

\begin{figure}[t]
        \centering
        \includegraphics[width=1.0\linewidth]{figures/3D-ISR_similarity_v2.pdf}
        \vspace{-4mm}
        % \includegraphics[width=\textwidth]{figures/3D-ISR.pdf}
        \caption{A visualization of the similarity score between text query and segmented 3D proposals. We compare sentence tokens used in ViL3DRel~\cite{chen2022language} with position embeddings used in 3D-ISR module.}
        \label{3d-isr-similarity}
        \vspace{-6mm}
\end{figure}

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figures/Visualization_all_tasks_v7.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% \vspace{-1mm}
\caption{Qualitative illustration of Inst3D-LMM across various 3D-language tasks in diverse 3D environments.} 
% Exemplary visualization results
\vspace{-4mm}
\label{all_tasks}
\end{figure*}




\subsection{3D Instance Spatial Relation (3D-ISR)}
Inspired by~\cite{chen2022language,zhu20233d,liangspatioawaregrouding3d}, we develop an effective 3D Instance Spatial Relation (3D-ISR) module to boost LLM's capabilities in assimilating spatial information within the 3D scene. 



ViL3DRel~\cite{chen2022language} uses language-conditioned self-attention to capture spatial relations in textual descriptions by feeding sentence tokens to update object tokens. However, as LLM is pre-trained on extensive textual data and requires fine-tuning on task-specific instructions, sentence tokens can introduce redundancy and hinder LLM's inherent ability. 


Inst3D-LMM extracts and integrates features at the instance level. 
Given that instances are sensitive to pairwise spatial relationships, we propose a spatial-conditioned self-attention mechanism. 
This mechanism incorporates position embeddings for each object along with pairwise spatial features to compute a spatial-conditioned attention map. The resulting attention map is then used to update the fused object tokens, to enhance spatial awareness. To minimize computational overhead and preserve the LLM's spatial understanding, we employ a scene projector to output a global scene feature via max pooling, as shown in Figure~\ref{3D-ISR}. We also provide a visualization, as shown in Figure~\ref{3d-isr-similarity}, of the similarity between the text query and segmented 3D proposals after processing by LLM. Compared to ViL3DRel~\cite{chen2022language} using sentence tokens, our 3D-ISR more accurately captures spatial relationships within the scene by employing position embeddings of objects.

3D-ISR utilizes the instance-level 3D visual tokens $\{O_{I1}^{3D},O_{I2}^{3D}, \ldots, O_{IN}^{3D}\}$ derived from MCMF module along with the corresponding center coordinates $\{C_{1},C_{2}, \ldots, C_{N}\}$ of all instances as inputs. For the $i$-th instance, we define its center coordinates as $C_i = \left(x_i,y_i,z_i\right)$.

For each pair of instance-level tokens $\{O_{Ii}^{3D},O_{Ij}^{3D}\}$, we calculate their Euclidean distance $d_{ij}=\left\| C_i - C_j \right\|_2$ as well as their horizontal angle $\theta_h$ and vertical angle $\theta_v$. Specially,  $\theta_h = \arctan2({{({y_j} - {y_i})} \mathord{\left/
 {\vphantom {{({y_j} - {y_i})} {({x_j} - {x_i})}}} \right.
 \kern-\nulldelimiterspace} {({x_j} - {x_i})}})$ and $\theta_v = \arcsin (({{{z_j} - {z_i})} \mathord{\left/
 {\vphantom {{{z_j} - {z_i})} {{d_{ij}}}}} \right.
 \kern-\nulldelimiterspace} {{d_{ij}}}})$. By making use of these positional parameters, we generate the pairwise spatial features $S=\{s_{ij}\} \in \mathbb{R}^{N \times N \times 5}$ as:
\begin{gather}
    s_{ij} = \left[\sin(\theta_h), \cos(\theta_h), \sin(\theta_v), \cos(\theta_v), d_{ij}\right].
\label{eq:spatial_features}
\end{gather}
%of the coordinates of object centers $C_i$ and $C_j$. 
% \begin{gather}



% \end{gather}

As illustrated in Figure~\ref{3D-ISR}, we create position embeddings $\mathcal{P}$ via the absolution positional encoding (PE), \textit{i.e.}  $\mathcal{P} = \text{PE}(C_{1},C_{2},\ldots,C_{N})$.
%the vanilla Positional Encoding layer in standard Transformer architecture. 
Next, we perform the spatial-conditioned self-attention operation. A spatial conditioned weight $l_i$ is computed to select the relevant spatial relations for each instance $O_{Ii}^{3D}$, which is formulated as below:
\begin{gather}
    % P = \text{PE}(C_{1},C_{2},\ldots,C_{n}),\\
    l_i = W_P^\top (\mathcal{P}_{i} + O_{Ii}^{3D}),
\end{gather}
where $W_P \in \mathbb{R}^{D \times 5}$ is a learnable parameter and the bias term is omitted for simplicity. The spatial condition attention map $\omega_{ij}$ is computed by combining $s_{ij}$, $l_i$ and $l_j$, \textit{i.e.} $\omega_{ij} = l_{i} \cdot s_{ij} \cdot l_{j}$.  
%as follows:
% \begin{equation}
%     \omega_{ij}^{s} = l_{i}^{s} \cdot f_{ij}^{s} \cdot l_{j}^{s}.
% \end{equation}
% Subsequently, the spatial condition attention map $\omega_{ij}$ is calculated by the sigmoid softmax function as follows:
% \begin{gather}
%     \omega_{ij} = \frac{\sigma(\omega_{ij}^{s}) \exp(w_{ij}^{v})}{\sum_{n=1}^{N} \sigma(\omega_{in}^{s}) \exp(w_{in}^{v})},
% \end{gather}
% where $\sigma(\cdot)$ is the sigmoid function. $w_{ij}^{v}$ is the vanilla self-attention weight. 

Through this positional transformation, the spatial condition attention map $\omega_{ij}$ encapsulates the pairwise spatial relationship across the entire 3D scene for each instance. We further integrate the attention map with instance-level visual tokens, which is formulated as below:
\begin{gather}
    % F = \text{Concat}(\sum_{j=1}^{N} \omega_{1j} O_{f1}^{3D}, \sum_{j=1}^{N} \omega_{2j} O_{f2}^{3D}, \ldots, \sum_{j=1}^{N} \omega_{Nj} O_{fN}^{3D}) \\
    F_i = \sum_{j=1}^{N} \omega_{ij} O_{Ii}^{3D}.
    % F_{scene} = \text{MLP}(\text{Encoder}(\text{Concat}(F_1, F_2, \ldots, F_N))).
\end{gather}
Finally, the instance-level representations are concatenated and further processed by a transformer-based encoder $\Gamma$, followed by a max-pooling layer (Pool) and a simple two-layer MLP. The scene-level relation-aware tokens $F_{scene} \in \mathbb{R}^{D}$ are generated 
% the instance-level token 
% outputs from the spatial condition self-attention and transformer-based encoder layers undergo a pooling layer to produce scene-level relation-aware tokens. 
% We adopt max-pooling since it can lead to better zero-shot visual grounding performance than average pooling. With the pooling layer and a simple two-layer MLP, 
% our 3D-ISR module can generate a spatial relation-aware token embedding
 for the entire 3D scene as follows:
\begin{gather}
    % F = \text{Concat}(\sum_{j=1}^{N} \omega_{1j} O_{f1}^{3D}, \sum_{j=1}^{N} \omega_{2j} O_{f2}^{3D}, \ldots, \sum_{j=1}^{N} \omega_{Nj} O_{fN}^{3D}) \\
    % F_i = \sum_{j=1}^{N} \omega_{ij} O_{Ii}^{3D},\\
    F_{scene} = \text{MLP}(\text{Pool}(\Gamma([F_1, F_2, \ldots, F_N]))).
\end{gather}

Thus,  we obtain the final token representations for LLM processing, \textit{i.e.} instance-level visual tokens $O_{Ii}^{3D}$ and spatial relation-aware tokens of the 3D scene $F_{scene}$, respectively.
% of  the $i$-th instance, denoted as $<\text{instance}[i]: O_{Ii}^{3D}, F_{scene}>$, where $O_{Ii}^{3D}$ and $F_{scene}$ represent the instance-aware visual token and .  


\subsection{End-to-End Multi-task Instruction Tuning}
\noindent \textbf{3D-Language Prompts.} Given an LMM, clear and explicit system messages and instructions are essential to support a range of downstream 3D vision-language tasks. 
For different tasks, we adopt various task-specific instruction templates with 3D features to generate uniform instruction data, enabling multi-task training. 
% We integrate text embeddings generated by a pre-trained tokenizer with instance-level attribute-aware tokens $\{O_{I1}^{3D},O_{I2}^{3D},\ldots,O_{IN}^{3D}\}$ and scene-level relation-aware tokens $F_{scene}$ to facilitate multi-task training. 
% For different downstream tasks, we utilize various system messages with different instructions. 
\textit{Please refer to the Supplementary Material for more detailed information.}
% regarding our utilized 3D-language prompts, please refer to the Supplementary Material.
% After obtaining all instance-level attribute-aware tokens $\{O_{I1}^{3D},O_{I2}^{3D},\ldots,O_{In}^{3D}\}$ and the global scene-level relation-aware tokens $F_{scene}$, we combine them  with text embeddings of system message and instructions to support various downstream tasks. F

\noindent \textbf{Instruction Tuning.} 
% The instruction fine-tuning dataset includes data conversation generated from various task-specific instruction templates. 
We conduct end-to-end multi-task fine-tuning 
% using the constructed 3D-language prompts that include data conversation generated from various task-specific instruction templates
to fully leverage the capabilities of our Inst3D-LMM framework. The MCMF and 3D-ISR modules enable the LLM with robust 3D scene understanding, grounding and reasoning abilities. We keep the pre-trained 3D object encoder frozen while updating both MCMF and 3D-ISR modules, as well as LLM.  
Upon completion of end-to-end multi-task instruction tuning, Inst3D-LMM can effectively handle various 3D vision-language tasks simultaneously, without fine-tuning on specific tasks, as illustrated in Figure~\ref{all_tasks}.
%In contrast to most existing methods that concentrate on close-set scene understanding or require task-specific fine-tuning, our instance-aware framework operates as a generalist model.

% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

==> sec/4_experiments-backup.tex <==
\section{Experiments}
\label{sec:experiments}
% In this section, we first introduce the details of our experimental setup. Then we benchmark our approach against leading methods quantitatively across various 3D scene understanding tasks. At the end of this section, the ablation analysis and qualitative results are presented.


% The entry of Inst3D-LMM (3D GT masks) denotes the use of 3D ground truth (GT) masks directly instead of predictions from a pre-trained 3D instance segmentation network (the same below).


\definecolor{mygreen}{RGB}{0, 128, 0}
\definecolor{myblue}{RGB}{108, 160, 220}
\definecolor{mygray}{gray}{0.6}
\begin{table*}[t]
    \setlength{\tabcolsep}{4.4pt}
    \centering
    \renewcommand\arraystretch{0.88}
    \scalebox{0.88}{%
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccc|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{Overall} & \multicolumn{2}{c}{Unique} & \multicolumn{2}{c|}{Multiple} & \multicolumn{2}{c}{Multi3DRefer} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
         & Acc@0.25\textuparrow & Acc@0.50\textuparrow & Acc@0.25\textuparrow & Acc@0.50\textuparrow & Acc@0.25\textuparrow & Acc@0.50\textuparrow & F1@0.25\textuparrow & F1@0.50\textuparrow \\
        \midrule
        \midrule
        \textbf{\textit{Closed-set, full sup.}} \\
        \textcolor{mygray}{ScanRefer \cite{chen2020scanrefer}} &  \textcolor{mygray}{37.3}& \textcolor{mygray}{24.3}& \textcolor{mygray}{65.0}&\textcolor{mygray}{43.3}& \textcolor{mygray}{30.6}&\textcolor{mygray}{19.8}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        
        \textcolor{mygray}{3DVG-Trans \cite{zhao20213dvg}} & \textcolor{mygray}{45.9}& \textcolor{mygray}{34.5}& \textcolor{mygray}{77.2}&\textcolor{mygray}{58.5}& \textcolor{mygray}{38.4}&\textcolor{mygray}{28.7}&\textcolor{mygray}{30.2}&\textcolor{mygray}{25.5}\\

        % \textcolor{mygray}{3DJCG \cite{zhao20213dvg}} & \textcolor{mygray}{49.6}& \textcolor{mygray}{37.3}& \textcolor{mygray}{83.5}&\textcolor{mygray}{64.3}& \textcolor{mygray}{41.4}&\textcolor{mygray}{30.8}&\textcolor{mygray}{31.4}&\textcolor{mygray}{26.6}\\

        % \textcolor{mygray}{D3Net \cite{chen2022d}} & \textcolor{mygray}{--}& \textcolor{mygray}{37.9}& \textcolor{mygray}{--}&\textcolor{mygray}{72.0}& \textcolor{mygray}{--}&\textcolor{mygray}{30.1}&\textcolor{mygray}{37.6}&\textcolor{mygray}{32.2}\\
        
        % \textcolor{mygray}{3D-VisTA \cite{zhu20233d}} &   \textcolor{mygray}{50.6}& \textcolor{mygray}{45.8}& \textcolor{mygray}{81.6}&\textcolor{mygray}{75.1}& \textcolor{mygray}{43.7}&\textcolor{mygray}{39.1}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\

        \textcolor{mygray}{M3DRef-CLIP \cite{zhang2023multi3drefer}} &  \textcolor{mygray}{51.9}& \textcolor{mygray}{44.7}& \textcolor{mygray}{--}&\textcolor{mygray}{77.2}& \textcolor{mygray}{--}&\textcolor{mygray}{36.8}&\textcolor{mygray}{42.8}&\textcolor{mygray}{38.4}\\
        % \textcolor{mygray}{EDA \cite{wu2023eda}} &  \textcolor{mygray}{54.6}& \textcolor{mygray}{42.3}& \textcolor{mygray}{85.8}&\textcolor{mygray}{68.6}& \textcolor{mygray}{49.1}&\textcolor{mygray}{37.6}&\\
        
        \textcolor{mygray}{ConcreteNet \cite{unal2023three}} &  \textcolor{mygray}{56.1}& \textcolor{mygray}{49.5}& \textcolor{mygray}{86.1}&\textcolor{mygray}{79.2}& \textcolor{mygray}{47.5}&\textcolor{mygray}{40.9}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        
        % \textcolor{mygray}{BUTD-DETR \cite{jain2022bottom}} & \textcolor{mygray}{52.2}& \textcolor{mygray}{39.8}& \textcolor{mygray}{84.2}&\textcolor{mygray}{66.3}& \textcolor{mygray}{46.6}&\textcolor{mygray}{35.1}&\\
        
       
        \textcolor{mygray}{CORE-3DVG \cite{yang2024exploiting}} & \textcolor{mygray}{56.8}& \textcolor{mygray}{43.8}& \textcolor{mygray}{85.0}&\textcolor{mygray}{67.1}& \textcolor{mygray}{51.8}&\textcolor{mygray}{39.8}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        \midrule
        \textbf{\textit{Zero-shot}} \\
        LLM-Grounder \cite{yang2023llm} & 17.1& 5.3& 30.8& 22.6&16.3&12.9&--&--\\
        Visual-Programming \cite{yuan2024visual} & 36.4& 32.7& \underline{63.8} & \underline{58.4} & \underline{27.7} & \underline{24.6}&--&--\\
        \midrule
        \textbf{\textit{Specialist}}\\
        OpenScene \cite{peng2023openscene} & 13.0& 5.1& 20.1& 13.1& 11.1& 4.4&--&--\\
        3D-LLM(Flamingo) \cite{hong20233d} & 21.2& --& --& --&--&--&--&--\\
        3D-LLM(BLIP2-flant5) \cite{hong20233d} & 30.3& --& --& --&--&--&--&--\\
        Chat-3D v2 \cite{huang2023chat} & 35.9& 30.4& 61.2& 57.6&25.2&22.6&45.1&41.6\\
         ReGround3D \cite{zhu2024empowering} & 53.1 & 41.1 & --& --&--&--&--&--\\
        \midrule
        \textbf{\textit{Generalist}}\\
        LAMM \cite{yin2024lamm} & --& 3.4& --& --&--&--&--&--\\
        3DMIT \cite{li20243dmit} & 10.7& 7.2& --& --&--&--&--&--\\
        Grounded 3D-LLM \cite{chen2024grounded} & 47.9 & 44.1 & --& --&--&--&45.2&40.6\\
        Chat-Scene \cite{huang2024chat} & \underline{55.5}& \underline{50.2}& -- & -- & -- & -- & \underline{57.1}&\underline{52.4}\\
        % \rowcolor{gray!12}
        % Inst3D-LMM(3D only) & 45.3& 41.2& 72.6 & 68.4 & 30.9 & 26.1 &46.2&41.3\\
        \rowcolor{gray!30}
        Inst3D-LMM  & \textbf{57.8} & \textbf{51.6} & \textbf{88.6} & \textbf{81.5}& \textbf{48.7} &\textbf{43.2}&\textbf{58.3}&\textbf{53.5}\\
        % \rowcolor{gray!12}
        % \textcolor{mygray}{Inst3D-LMM (3D GT masks)} & \textcolor{mygray}{54.8} & \textcolor{mygray}{48.0} & \textcolor{mygray}{85.7} & \textcolor{mygray}{79.2}& \textcolor{mygray}{47.6} &\textcolor{mygray}{40.2}&\textcolor{mygray}{52.6}&\textcolor{mygray}{48.7}\\
        \bottomrule
    \end{tabular}
    }
    % }
     \vspace{-2mm}
    \caption{Quantitative results for 3D Visual Grounding on ScanRefer and Multi3DRefer validation sets. In the ScanRefer dataset, scenes are labeled as ``unique" (one object per class) or ``multiple" (more than one).
    Closed-set methods are fully supervised for specific datasets.
    ``Zero-shot" refers to methods that directly use LLMs without fine-tuning. ``Specialist" and ``Generalist" categorize methods fine-tuned for specific tasks versus those trained jointly. \textbf{Bold} and \underline{underlined} numbers indicate the best and the second-best results, respectively.}
    \label{tab:scanrefer}
    \vspace{-1mm}
\end{table*}

\begin{table*}[t]
    \centering
    % \resizebox{\textwidth}{!}{%
    \scalebox{0.785}{%
    \begin{tabular}{lccccccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{\makecell{\# 3D Data \\ for Alignment}}  & \multicolumn{6}{c}{ScanQA} & \multicolumn{4}{c}{Scan2Cap@0.50}\\
        \cmidrule(lr){3-8} \cmidrule(lr){9-12}
        &   & B-1\textuparrow & B-4\textuparrow & METEOR\textuparrow & ROUGE\textuparrow &  CIDER\textuparrow & EM\textuparrow & B-4\textuparrow & METEOR\textuparrow & ROUGE\textuparrow & CIDER\textuparrow  \\
        
        \midrule
        \midrule
        \textbf{\textit{Closed-set, full sup.}}\\
         % \textcolor{mygray}{VoteNet \cite{ding2019votenet} + MCAN \cite{yu2019deep}} &  \textcolor{mygray}{--} &  \textcolor{mygray}{28.0}& \textcolor{mygray}{6.2}& \textcolor{mygray}{11.4}&\textcolor{mygray}{29.8}& \textcolor{mygray}{54.7}&\textcolor{mygray}{17.3}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        \textcolor{mygray}{VoteNet \cite{ding2019votenet} + MCAN \cite{yu2019deep}} &  \textcolor{mygray}{--} &  \textcolor{mygray}{28.0}& \textcolor{mygray}{6.2}& \textcolor{mygray}{11.4}&\textcolor{mygray}{29.8}& \textcolor{mygray}{54.7}&\textcolor{mygray}{17.3}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\

        % \textcolor{mygray}{ScanRefer \cite{chen2020scanrefer} + MCAN \cite{yu2019deep}} & \textcolor{mygray}{--} &  \textcolor{mygray}{26.9}& \textcolor{mygray}{7.9}& \textcolor{mygray}{11.5}&\textcolor{mygray}{30.0}& \textcolor{mygray}{55.4}&\textcolor{mygray}{18.6}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        \textcolor{mygray}{ScanRefer \cite{chen2020scanrefer} + MCAN \cite{yu2019deep}} & \textcolor{mygray}{--} &  \textcolor{mygray}{26.9}& \textcolor{mygray}{7.9}& \textcolor{mygray}{11.5}&\textcolor{mygray}{30.0}& \textcolor{mygray}{55.4}&\textcolor{mygray}{18.6}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\

        \textcolor{mygray}{ScanQA \cite{chen2021scan2cap}} & \textcolor{mygray}{--} &  \textcolor{mygray}{30.2}& \textcolor{mygray}{10.1}& \textcolor{mygray}{13.1}&\textcolor{mygray}{33.3}& \textcolor{mygray}{64.9}&\textcolor{mygray}{21.0}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{--}\\
        
        \textcolor{mygray}{Scan2Cap \cite{azuma2022scanqa}}  & \textcolor{mygray}{--} &  \textcolor{mygray}{--}& \textcolor{mygray}{--}& \textcolor{mygray}{--}&\textcolor{mygray}{--}& \textcolor{mygray}{--}&\textcolor{mygray}{--}&\textcolor{mygray}{22.4}&\textcolor{mygray}{21.4}&\textcolor{mygray}{43.5}&\textcolor{mygray}{35.2}\\
        
        \textcolor{mygray}{3D-VisTA \cite{zhu20233d}}  & \textcolor{mygray}{--} &  \textcolor{mygray}{34.2}& \textcolor{mygray}{13.1}& \textcolor{mygray}{15.2}&\textcolor{mygray}{38.6}& \textcolor{mygray}{76.6}&\textcolor{mygray}{27.0}&\textcolor{mygray}{34.0}&\textcolor{mygray}{27.1}&\textcolor{mygray}{54.3}&\textcolor{mygray}{66.9}\\        
        \midrule
        \textbf{\textit{LLM-based Methods}}\\
        LLaVA (zero-shot) \cite{liu2024visual} &  -- &  7.1 & 0.3& 10.5 & 12.3 & 5.7 & 0.2 & 1.5 & 8.3 & 19.6&3.2  \\
        LAMM \cite{yin2024lamm}  & 25K & 26.8& 5.8& 10.0& 23.6&42.4&9.8&--&--&--&--\\
        3D-LLM(Flamingo) \cite{hong20233d}  & 675K & 30.3& 7.2& 12.2& 32.3&59.2&20.4&5.9&11.4&29.9&--\\
        3D-LLM(BLIP2-flant5) \cite{hong20233d}  & 675K & \underline{39.3} & 12.0& 14.5& 35.7&69.4&20.5&8.1&13.1&33.2&--\\
        Chat-3D v2 \cite{huang2023chat}  & 38K & 38.4& 7.3& \underline{16.1}& \underline{40.1}&77.1&\underline{21.1}& 31.8 & 22.3 & 50.2&63.9\\
        LL3DA \cite{chen2024ll3da}  & 38K & --& 13.3& 15.4 & 37.0 & 75.7&--& 35.9 & \underline{25.6} & \underline{54.6}&65.2 \\
        Grounded 3D-LLM \cite{chen2024grounded}  & 107K & --& 13.4 & --& --&72.7&--&  35.5 & -- & -- & 70.6 \\
        Chat-Scene \cite{huang2024chat}  & 38K & -- & \underline{14.3} & -- & --
 &\underline{87.7}& -- & \underline{36.3} & -- & -- &\underline{77.1}\\
         % \rowcolor{gray!12}
        % \rowcolor{gray!12}
        % Inst3D-LMM(3D only) & 38K & 39.1& 7.8& 15.7& 37.4&72.3&18.2&  30.8 & 25.8 & 52.4& 64.3 \\
        \rowcolor{gray!30}
        Inst3D-LMM  & 38K & \textbf{43.5} & \textbf{14.9} & \textbf{18.4} & \textbf{42.6} & \textbf{88.6} & \textbf{24.6} &  \textbf{38.3} & \textbf{27.5} & \textbf{57.2}&\textbf{79.7} \\
        % \rowcolor{gray!12}
        % \textcolor{mygray}{Inst3D-LMM (3D GT masks)} &\textcolor{mygray}{38K} &\textcolor{mygray}{46.7} & \textcolor{mygray}{17.8} & \textcolor{mygray}{21.5} & \textcolor{mygray}{45.9}& \textcolor{mygray}{88.6} &\textcolor{mygray}{27.2}&\textcolor{mygray}{41.5}&\textcolor{mygray}{29.4}&\textcolor{mygray}{57.1}&\textcolor{mygray}{75.3}\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-1mm}
    \caption{Quantitative results for 3D Question Answering and 3D Dense Captioning on the ScanQA and Scan2Cap datasets.}
    \label{tab:scanqa}
    \vspace{-3.0mm}
\end{table*}

\subsection{Experimental Setting}
\noindent \textbf{Datasets and Benchmarks.} In this work, we conduct our experiments on the ScanNetv2 dataset \cite{dai2017scannet}, an extensive indoor 3D scene dataset comprising 1,513 scenes. This dataset includes 3D point clouds, RGB-D frames, and detailed point-level instance segmentation annotations. 
The whole dataset is divided into 1,201 scenes for training and 312 scenes for validation, with all subsequent benchmarks adhering to these training/validation splits. 
Our evaluation encompasses a range of 3D scene understanding benchmarks, including ScanRefer \cite{chen2020scanrefer} and Multi3DRefer \cite{zhang2023multi3drefer} for single- and multi-object 3D Visual Grounding, respectively, ScanQA \cite{azuma2022scanqa} for 3D Question Answering, and Scan2Cap \cite{chen2021scan2cap} for 3D Dense Captioning. These datasets are converted into a uniform instruction format for multi-task instruction tuning and performance assessment.


\noindent \textbf{Implementation Details.} For 3D feature extraction, we leverage the 3D instance segmentation model Mask3D~\cite{schult2023mask3d} pre-trained on ScanNet200 dataset~\cite{rozenberszki2022language}, alongside the 3D object encoder Ulip2~\cite{xue2023ulip2}/Uni3D~\cite{zhou2023uni3d} based on ViT-L/14~\cite{dosovitskiy2020image}. 
For 2D feature extraction, we adopt the ViT-H-based SAM~\cite{kirillov2023segment} to obtain high-quality masks. Moreover, we exact  2D semantic features using the vision encoder from CLIP-ViT-L/14-336px~\cite{radford2021learning}. These pre-trained models are kept frozen.
In our method, we apply multi-view selection and multi-level crops to 2D images, setting $K=5$ views and $L=3$ levels. We use Vicuna1.5-7B \cite{chiang2023vicuna} as our basic LLM, which is fine-tuned from LLaMA2 \cite{touvron2023llama}. 
Our fine-tuning process utilizes LoRA \cite{hu2021lora}. We adopt the AdamW optimizer with a weight decay of 0.02. All experiments are conducted on 8 NVIDIA A100 GPUs.


\subsection{Main Results}
\noindent \textbf{3D Visual Grounding.} 
We first report the visual grounding performance on ScanRefer and Multi3DRefer validation datasets. As shown in Table~\ref{tab:scanrefer}, our approach outperforms the state-of-the-art model, Chat-Scene~\cite{huang2024chat}, by \textcolor{mygreen}{+2.3}\% Acc@0.25 and \textcolor{mygreen}{+1.2}\% F1@0.25 on ScanRefer and Multi3DRefer, respectively. Compared to Specialist and closed-set methods, Inst3D-LMM, \textit{trained with a generalist approach}, achieves competitive performance. Figure~\ref{small-vg} displays typical visual comparison results.\\
% By utilizing 3D GT masks rather than predictions from a pre-trained network, our approach shows significant improvements, which further validate the effectiveness of our framework.
\noindent \textbf{3D Question Answering.} We then compare  Inst3D-LMM with previous leading methods on the ScanQA validation set. Table~\ref{tab:scanqa} reports the results. Our Inst3D-LMM consistently outperforms these methods, including the recent LL3DA~\cite{chen2024ll3da}, Grounded 3D-LLM~\cite{chen2024grounded} and Chat-Scene~\cite{huang2024chat}.\\
% Similarly, our method obtains consistent performance gains using 3D ground-truth masks.
\noindent \textbf{3D Dense Captioning.} This task involves the localization and description of instances. As shown in Table~\ref{tab:scanqa}, our approach achieves 38.3\% B-4@0.50 and 79.7\% C@0.50 on Scan2Cap, which  exceeds the closed-set expert model 3D-VisTA~\cite{zhu20233d} by \textcolor{mygreen}{+4.3}\% and \textcolor{mygreen}{+12.8}\%, and still outperforms LLM-based method LL3DA by \textcolor{mygreen}{+2.4}\% and \textcolor{mygreen}{+14.5}\%.


\begin{figure}[t]
        \centering
        \includegraphics[width=1.0\linewidth]{figures/small_Visualization_VG.pdf}
        \vspace{-4mm}
        % \includegraphics[width=\textwidth]{figures/3D-ISR.pdf}
        \caption{Visual comparisons in 3D Visual Grounding. The rendered images show the ground-truth (\textcolor{blue}{blue}), incorrectly identified objects (\textcolor{red}{red}), and correctly identified objects (\textcolor{green}{green}). The colored text indicates the results of text decoupling.}
        \label{small-vg}
        \vspace{-5.0mm}
\end{figure}

\subsection{Ablation Study}
In this section, we perform ablation experiments to thoroughly evaluate the effectiveness of components. \textit{Please refer to the Supplementary Material for more analysis.} \\
\textbf{Effects of Multi-view Cross-Modal Fusion (MCMF).} The MCMF module aims to augment LLM's understanding of 3D instances' geometric and semantic attributes. We explore several methods to combine these features, including direct concatenation for projection (`Concat.'), parallel projection followed by combination (`Parallel'), and vanilla cross-attention (`Cross-Attention'). To encode the basic spatial information, we concatenate the results of absolution positional encoding (PE) with the 3D features. As shown in Table~\ref{tab:ablation_MCMF},  MCMF outperforms all these methods on ScanRefer, ScanQA and Scan2Cap datasets. We also observe that the performance of 3D LMM is significantly improved by incorporating multi-view 2D CLIP information compared to using only 3D geometric features. These results demonstrate the effectiveness of our MCMF approach.



% +



\begin{table}[h]
\vspace{-2mm}
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|cccccccccc}
\toprule
% \hline 
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{ScanQA} & \multicolumn{2}{c}{Scan2Cap@0.50} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                    &Acc@0.25\textuparrow & Acc@0.50\textuparrow & B-1\textuparrow & CIDER\textuparrow & B-4\textuparrow & CIDER\textuparrow \\ 
                    \midrule \midrule
                    % \hline\hline
\textit{w/o} Multi-view 2D & 36.0 & 31.9 & 31.5 & 57.3 & 19.9 & 54.3  \\ 
 Concat. & 38.8 & 34.4 & 36.6 & 65.4 & 25.2 & 63.3\\ 
 Parallel & 37.6 & 33.5 & 35.3 & 63.9 & 24.8 & 62.1  \\ 
 Cross-Attention & 39.2 & 36.5 & 37.4 & 66.1 & 25.5 & 64.3  \\
 \rowcolor{gray!30}
 MCMF & \textbf{46.7} & \textbf{41.9} & \textbf{41.5} & \textbf{78.6} & \textbf{32.7} & \textbf{68.2} \\
% MCMF + 3D-ISR (full) & \textbf{43.5} & \textbf{18.4} & \textbf{42.6} & \textbf{86.5} & \textbf{36.2} & \textbf{26.2} & \textbf{55.5} & \textbf{70.8} \\
\bottomrule
% \hline
\end{tabular}
}
\vspace{-1.5mm}
\caption{Ablation evaluations of the proposed Multi-view Cross-Modal Fusion (MCMF) module.}
\vspace{-4mm}
\label{tab:ablation_MCMF}
\end{table}

\begin{figure}[t]
        \centering
        \includegraphics[width=1.0\linewidth]{figures/3D-ISR_similarity-new.pdf}
        \vspace{-4mm}
        % \includegraphics[width=\textwidth]{figures/3D-ISR.pdf}
        \caption{A visualization of the similarity score between text query and segmented 3D proposals. We compare sentence tokens used in ViL3DRel~\cite{chen2022language} with position embeddings employed in 3D-ISR.}
        \label{3d-isr-similarity}
        \vspace{-5mm}
\end{figure}


\begin{figure*}[t]
\centering
\includegraphics[width=0.98\linewidth]{figures/Visualization_all_tasks-new.pdf} % Reduce the figure size so that it is slightly narrower than the column.
\vspace{-1mm}
\caption{Qualitative illustration of Inst3D-LMM across various 3D-language tasks in diverse 3D environments.} 
% Exemplary visualization results
\vspace{-4mm}
\label{all_tasks}
\end{figure*}


\noindent \textbf{Impacts of 3D Instance Spatial Relation (3D-ISR).} We further investigate 3D-ISR module to analyze its impact on 3D spatial understanding using only 3D geometry priors.
We compare 3D-ISR against previous spatial relation modeling methods, such as the 3D localization mechanism in ViL3DRel~\cite{chen2022language} and 3D-LLM~\cite{hong20233d}, and relation-aware token generation in Chat-3D-v2~\cite{huang2023chat}. Table~\ref{tab:ablation_3D-ISR} reports the comparison results. It can be observed that our 3D-ISR consistently surpasses these approaches.
% As shown in Table~\ref{tab:ablation_3D-ISR}, our 3D-ISR strategy outperforms other relation modules proposed in various works. 
Specifically, 3D-ISR significantly enhances performance on grounding tasks (ScanRefer and Multi3dRefer). This aligns with the motivation of our design.  We also provide a visualization, as shown in Figure~\ref{3d-isr-similarity}, of the similarity between the text query and segmented 3D proposals after processing by LLM. Compared to ViL3DRel~\cite{chen2022language} using sentence tokens, our 3D-ISR more accurately captures spatial relationships within the scene by employing position embeddings of objects.
% It indicates that the 3D-ISR module enables LLMs to understand the intricate spatial details in 3D scenes so that their localization capabilities can be enhanced.
\begin{table}[h]
\vspace{-2.0mm}
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{Multi3DRefer} & \multicolumn{2}{c}{ScanQA} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                     & Acc@0.25\textuparrow    & Acc@0.50\textuparrow & F1@0.25\textuparrow  & F1@0.50\textuparrow    & B-1\textuparrow & CIDER\textuparrow   \\ \midrule \midrule
\textit{w/o} spatial relation & 35.6 & 29.8 & 34.8 & 27.3 & 29.2 & 55.6 \\
 ViL3DRel \cite{chen2022language}& 36.1 & 30.5 & 38.4 & 35.5 & 32.8 & 58.9 \\
 3D-LLM \cite{hong20233d} & 39.2 & 36.8 & 42.4 & 35.2 & 32.5 & 60.2 \\ 
 Chat-3D-v2 \cite{huang2023chat}& 40.8 & 37.5 & 41.6 & 37.8 & 35.1 & 64.6  \\ 
 \rowcolor{gray!30}
 3D-ISR  & \textbf{48.3} & \textbf{44.1} & \textbf{46.2} & \textbf{41.3} & \textbf{39.1} & \textbf{72.3}  \\
% MCMF + 3D-ISR (full) & \textbf{49.6} & \textbf{45.7} & \textbf{49.8} & \textbf{46.4} & \textbf{43.5} & \textbf{86.5}  \\
\bottomrule
\end{tabular}
}
\vspace{-2.5mm}
\caption{Ablation study to verify the effectiveness of our 3D Instance Spatial Relation (3D-ISR) module.}
\vspace{-3mm}
\label{tab:ablation_3D-ISR}
\end{table}







\noindent \textbf{Ablations within MCMF and 3D-ISR modules.} We also explore the effectiveness of key designs in MCMF and 3D-ISR modules. The learnable \texttt{[CLS]} token in the MCMF module is introduced to aggregate 2D multi-view features. We compare it against alternative methods, such as token max pooling and Q-Former~\cite{li2023blip}.  Table~\ref{tab:ablation_cls_token} reports the comparison results, demonstrating the efficacy of the learnable \texttt{[CLS]} token design. Besides, to assess the impact of different pairwise spatial features in the 3D-ISR module, we evaluate the model using only distance or orientation information to compute spatial features in Eq~\ref{eq:spatial_features}. Results in Table~\ref{tab:ablation_in_3D-ISR} reveal that distance has a greater impact on the model's grounding capability, while orientation is more crucial in handling Q\&A tasks. Combining both pairwise distance and orientation yields the best overall performance.
% across various benchmarks.









\noindent \textbf{Mutual Benefits of MCMF and 3D-ISR.} As shown in Table~\ref{tab:collaboration}, the model integrating both MCMF and 3D-ISR consistently outperforms those utilizing either module alone across multiple tasks. To further verify its effectiveness, we combine MCMF with absolution positional encoding (PE) for the basic spatial relation, and directly adopt feature concatenation (Concat.) to integrate  3D object features and 2D multi-view features along with 3D-ISR. These results indicate the synergy efforts between MCMF and 3D-ISR. 
% in Inst3D-LMM.  
% enhances the performance of our Inst3D-LMM. 


\begin{table}[t]
% \vspace{-2mm}
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|cccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{ScanQA} & \multicolumn{2}{c}{Scan2Cap@0.50} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                    &Acc@0.25\textuparrow & Acc@0.50\textuparrow & B-1\textuparrow & CIDER\textuparrow & B-4\textuparrow & CIDER\textuparrow \\ \midrule \midrule
Max Pooling & 48.7 & 44.6 & 39.2 & 74.8 & 30.6 & 65.5 \\ 
Q-Former~\cite{li2023blip} & 53.2 & 47.9 & \textbf{44.3} & 87.9 & 35.4 & 78.6  \\ 
\rowcolor{gray!30}
CLS Token & \textbf{57.8} & \textbf{51.6} & 43.5 & \textbf{88.6} & \textbf{38.3} & \textbf{79.7} \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Ablation study of learnable CLS token in MCMF module.}
\vspace{-3.5mm}
\label{tab:ablation_cls_token}
\end{table}

\begin{table}[t]
% \vspace{-2.0mm}
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{Multi3DRefer} & \multicolumn{2}{c}{ScanQA} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                     & Acc@0.25\textuparrow    & Acc@0.50\textuparrow & F1@0.25\textuparrow  & F1@0.50\textuparrow    & B-1\textuparrow & CIDER\textuparrow   \\ \midrule \midrule
\textit{w/} Dist (only) & 43.2 & 38.0 & 42.4 & 37.8 & 31.2 & 65.7 \\
 \textit{w/} Ort (only) & 39.7 & 33.6 & 40.5 & 35.9 & 32.5 & 66.8 \\
 \rowcolor{gray!30}
 Dist + Ort & \textbf{48.3} & \textbf{44.1} & \textbf{46.2} & \textbf{41.3} & \textbf{39.1} & \textbf{72.3} \\ 
\bottomrule
\end{tabular}
}
\vspace{-1.5mm}
\caption{Ablation study of 3D-ISR module. Dist (Ort) means only using distance (orientation) to compute pairwise spatial features.}
\vspace{-5.5mm}
\label{tab:ablation_in_3D-ISR}
\end{table}







\noindent \textbf{Different LLMs and Foundation Models.} Table~\ref{tab:ablation_LLM_mini} presents  the results of various LLMs and pre-trained 2D/3D models, including Vicuna-7B~\cite{chiang2023vicuna} \textit{vs} Vicuna-13B, Ulip2~\cite{xue2023ulip2} \textit{vs} Uni3D~\cite{zhou2023uni3d}, CLIP~\cite{radford2021learning} \textit{vs} SigLIP~\cite{mu2022slip}, and ViT-H-based SAM~\cite{kirillov2023segment} \textit{vs} ViT-L-based SAM. We find that the performance of grounding and reasoning increases along with the total number of parameters in the foundation models (\textit{i.e.} ViT-L \textit{vs} Vit-H and 7B \textit{vs} 13B). These results indicate that our framework's capabilities can be improved in tandem with the performance of foundation models. 
% \textbf{Training Time and Memory Usage.} Here we compare the training time and graphics memory usage with and without the incorporation of multi-view 2D image information. As shown in Table~\ref{tab:ablation_time&mem}, our model, based on both two LLMs, does not exhibit a significant increase in training time or computational resource expenditure, which demonstrates the feasibility of our proposed framework. 


\begin{table}[t]
% \vspace{-3mm}
\centering
\resizebox{0.472\textwidth}{!}{%
\begin{tabular}{c|cccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{ScanQA} & \multicolumn{2}{c}{Scan2Cap@0.50} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                     & Acc@0.25\textuparrow    & Acc@0.50\textuparrow & B-1\textuparrow & CIDER\textuparrow & B-4\textuparrow & CIDER\textuparrow  \\ \midrule\midrule
\textit{w/} MCMF (only)& 38.2 & 34.6 & 39.4 & 76.8 & 30.5 & 66.9\\
\textit{w/} 3D-ISR (only) & 48.3 & 44.1 & 39.1 & 72.3 & 29.8 & 64.3\\
MCMF + PE & 46.7 & 41.9 & 41.5 & 78.6 & 32.7 & 68.2 \\
3D-ISR + Concat. & 49.8 & 45.0 & 40.6 & 75.4 & 33.3 & 66.5 \\
\rowcolor{gray!30}
MCMF + 3D-ISR (full) & \textbf{57.8} & \textbf{51.6} & \textbf{43.5} & \textbf{88.6} & \textbf{38.3} & \textbf{79.7}\\
\bottomrule
\end{tabular}
}
\vspace{-1.5mm}
\caption{Comparison results of the collaboration between MCMF and 3D-ISR modules.}
\vspace{-4mm}
\label{tab:collaboration}
\end{table}




\begin{table}[t]
% \vspace{-3mm}
\centering
\resizebox{0.472\textwidth}{!}{
\begin{tabular}{c|c|c|cccc}
\toprule
% \multirow{2}{*}{Method} &\multirow{2}{*}{Model} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{4}{c}{ScanQA} \\
\multirow{2}{*}{LLM} & \multirow{2}{*}{3D Encoder} & \multirow{2}{*}{2D VFMs} & \multicolumn{2}{c}{ScanRefer} & \multicolumn{2}{c}{ScanQA} \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} 
 & &  & Acc@0.25\textuparrow & Acc@0.50\textuparrow & B-1\textuparrow & CIDER\textuparrow \\ \midrule\midrule
% \cmidrule(lr){3-4} \cmidrule(lr){5-8}
%                     & & Acc@0.25    & Acc@0.50 & B-1  & METEOR    & ROUGE & CIDER   \\ \midrule
% Ours(LLaVA1.5-7b) & Ulip2 & 42.2 & 12.9 & 18.1 & 40.4 & 86.2 & 20.8  \\ 
% Ours(LLaVA1.5-7b) & Uni3D & 41.8 & 13.4 & 17.8 & 41.6 & 87.8 & 21.5  \\ \midrule
Vicuna-7B & Ulip2 & CLIP+SAM (ViT-L) & 49.2 & 44.8 & 39.5 & 79.6 \\
Vicuna-7B & Ulip2 & CLIP+SAM (ViT-H) & 53.6 & 46.5 & \textbf{43.7} & 87.5 \\
Vicuna-7B & Ulip2 & SigLIP+SAM (ViT-H) & 54.3 & 47.0 & 42.2 & 84.5\\ \midrule
\rowcolor{gray!30}
Vicuna-7B & Uni3D & CLIP+SAM (ViT-H) & \textbf{57.8} & 51.6 & 43.5 & \textbf{88.6}\\
Vicuna-13B & Uni3D & CLIP+SAM (ViT-H) & 56.0 & \textbf{52.0} & 42.8 & 83.1 \\
Vicuna-13B & Uni3D & SigLIP+SAM (ViT-H) & 55.2 & 47.8& 43.3 & 85.4\\
\bottomrule
\end{tabular}
}
\vspace{-1.5mm}
\caption{Ablation study of different LLMs and pre-trained foundation models.}
\vspace{-5.5mm}
\label{tab:ablation_LLM_mini}
\end{table}

% \begin{table}[h]
% \centering
% \resizebox{0.47\textwidth}{!}{%
% \begin{tabular}{c|c|cc}
% \toprule
% {Method} & LLM & {VRAM per GPU\textdownarrow} & {Training Time\textdownarrow} \\ 
% \midrule\midrule
% LEO \cite{huang2023leo} & Vicuna-7B & $\sim$80 GB  & $\sim$42 hours \\
% LL3DA \cite{chen2024ll3da} & OPT-6.7B & $\sim$60 GB  & $\sim$36 hours  \\
% Chat-Scene \cite{huang2024chat} & Vicuna-7B & $\sim$70 GB& $\sim$8 hours \\
% \rowcolor{gray!20}
% Inst3D-LMM (3D only) & Vicuna-7B & $\sim$50 GB & $\sim$3.5 hours\\ 
% \rowcolor{gray!20}
% Inst3D-LMM (3D+2D) & Vicuna-7B &$\sim$55 GB & $\sim$ 4 hours\\ 
% \bottomrule
% \end{tabular}
% }
% \vspace{-1.5mm}
% \caption{Comparison of training time and memory usage between Inst3D-LMM and other methods.}
% \vspace{-4mm}
% \label{tab:compare_time&mem}
% \end{table}


